On the structure of tensor products of the finite-dimensional representations of quantum affine $\mathfrak{sl}_n$

We review some important facts about the structure of tensor products of finite dimensional representations of quantum affine algebras. This is done from the elementary standpoint of the representation theory of semisimple Lie algebras in the scope of a masters thesis. We set the focus on drawing the line to the finite dimensional representation theory of quantum affine $\mathfrak{sl}_n$, the theory of q-characters, and introduce the so called snake modules together with their character formula.

==> Erklaerung_Thesis.tex <==
\newpage
\thispagestyle{empty}
\begin{otherlanguage}{ngerman}
\begin{center}
	\textbf{Erklärung}\\
	gem. §15 Abs. 6 Prüfungsordnung vom 13.11.2019\\
\end{center}         
Hiermit erkläre ich, Henrik Jürgens, dass ich die von mir eingereichte Abschlussarbeit (Master-Thesis) mit dem Titel\\


"`\sisetup{detect-weight=true,detect-inline-weight=math}\textbf{On the structure of tensor products of the finite-dimensional representations of quantum affine} $\boldsymbol{\mathfrak{sl}_n}$"'\\ 


selbstständig verfasst und keine anderen als die angegebenen Quellen und Hilfsmittel benutzt sowie Stellen der Abschlussarbeit, die anderen Werken dem Wortlaut oder Sinn nach entnommen wurden, in jedem Fall unter Angabe der Quelle als Entlehnung kenntlich gemacht habe.

\vspace{2cm}

\begin{tabular}{lp{18em}l}
	Wuppertal, 04.09.2024    && \hspace{3cm} \\\cline{1-1}\cline{3-3}
	Ort, Datum     && Unterschrift
\end{tabular}


\vspace{3cm}

\begin{center}
	\textbf{Erklärung}
\end{center}
Hiermit erkläre ich, Henrik Jürgens, mich damit einverstanden, dass meine Abschlussarbeit (Master-Thesis) wissenschaftlich interessierten Personen oder Institutionen und im Rahmen von externen Qualitätssicherungsmaßnahmen des Studienganges zur Einsichtnahme zur Ver\-fügung gestellt werden kann.\\
Korrektur- oder Bewertungshinweise in meiner Arbeit dürfen nicht zitiert werden.

\vspace{2cm}

\begin{tabular}{lp{18em}l}
	Wuppertal, 04.09.2024    && \hspace{3cm} \\\cline{1-1}\cline{3-3}
	Ort, Datum     && Unterschrift
\end{tabular}
\end{otherlanguage}
